Stabilising and accelerating light gated recurrent units for automatic speech recognition

The light gated recurrent units (Li-GRU) is well-known for achieving impressive results in automatic speech recognition (ASR) tasks while being lighter and faster to train than a standard gated recurrent units (GRU). However, the unbounded nature of its rectified linear unit on the candidate recurrent gate induces an important gradient exploding phenomenon disrupting the training process and preventing it from being applied to famous datasets. In this paper, we theoretically and empirically derive the necessary conditions for its stability as well as engineering mechanisms to speed up by a factor of five its training time, hence introducing a novel version of this architecture named SLi-GRU. Then, we evaluate its performance both on a toy task illustrating its newly acquired capabilities and a set of three different ASR datasets demonstrating lower word error rates compared to more complex recurrent neural networks.

==> resources/curve_benchmark.tex <==

\begin{figure*}[!th]
\begin{center}
\scalebox{0.94}{
\begin{tabular}{c c}

\multicolumn{1}{c}{
\begin{tikzpicture}
\begin{axis}[
    name=ax1,
    width=9cm, height=5cm,   % size of the image
    grid = major,
    grid style={dashed, gray!30},
    xmin=100,   % start the diagram at this x-coordinate
    xmax=9000,  % end  the diagram at this x-coordinate
    ymin=0,   % start the diagram at this y-coordinate
    ymax=1.5,  % end  the diagram at this y-coordinate
    axis background/.style={fill=white},
    tick align=outside,
    xtick={100, 1500 , 3000, 4500, 6000, 7500, 9000, 9500},
    ytick={0, 0.25, 0.5, 0.75, 1, 1.25, 1.5},
    mark repeat={600},
    ylabel near ticks,
    ylabel={Time in Seconds},
    xlabel near ticks,
    xlabel style={text width=5cm},
    xlabel style={align=center},
    xlabel={Sequence Length},
    title={Forward Propagation},
    legend to name=leg,
    legend columns=4,
    %legend style={at={(1,-0.5)},anchor=north,legend cell align=left,legend columns=5}
    %legend style={font=\small, at={(0,-0.1)},anchor=north east,legend columns=5},
    ]

\addplot+[mark=none,color=purple,line width=1pt] file {resources/dataset/benchmark/inference/ligru_jit.txt};%\addlegendentry{ASR $\rightarrow$ ASR}
\addlegendentry{Li-GRU}

\addplot+[mark=none,color=green, dash pattern=on 3pt off 4pt on 5pt off 5pt, line width=1pt] file {resources/dataset/benchmark/inference/ligru_2_0_cudnn.txt};%\addlegendentry{ASR $\rightarrow$ ASR}
\addlegendentry{Li-GRU 2.0}

\addplot+[mark=none,color=orange, line width=1pt] file {resources/dataset/benchmark/inference/lstm_cudnn.txt};%\addlegendentry{ASR $\rightarrow$ ASR}
\addlegendentry{LSTM}



%/ LiGRU 16M / LSTM 33M = 4 Layers 1024 Neurons
%/ LiGRU 33M = 4 Layers 1480 Neurons

\end{axis}
\end{tikzpicture}
}

& 
\multicolumn{1}{c}{
\begin{tikzpicture}
\begin{axis}[
    at={(ax1.south east)},
    xshift=2cm,
    width=9cm, height=5cm,   % size of the image
    grid = major,
    grid style={dashed, gray!30},
    xmin=100,   % start the diagram at this x-coordinate
    xmax=9000,  % end  the diagram at this x-coordinate
    ymin=0,   % start the diagram at this y-coordinate
    ymax=3,  % end  the diagram at this y-coordinate
    axis background/.style={fill=white},
    tick align=outside,
    xtick={100, 1500 , 3000, 4500, 6000, 7500, 9000},
    ytick={0, 0.5, 1., 1.5, 2, 2.5, 3},
    mark repeat={600},
    ylabel near ticks,
    ylabel={Time in Seconds},
    xlabel near ticks,
    xlabel style={text width=5cm},
    xlabel style={align=center},
    xlabel={Sequence Length},
    title={Backward Propagation}
]

%     legend style={font=\small, at={(0.01, -0.35)},anchor=north east,legend columns=3} 
\addplot+[mark=none,color=purple,line width=1pt] file {resources/dataset/benchmark/backward/ligru_jit.txt};%\addlegendentry{ASR $\rightarrow$ ASR}
\addlegendentry{Li-GRU}

\addplot+[mark=none,color=green, dash pattern=on 3pt off 4pt on 5pt off 5pt, line width=1pt] file {resources/dataset/benchmark/backward/ligru_2_0_cudnn.txt};%\addlegendentry{ASR $\rightarrow$ ASR}
\addlegendentry{Li-GRU 2.0}

\addplot+[mark=none,color=orange, line width=1pt] file {resources/dataset/benchmark/backward/lstm_cudnn.txt};%\addlegendentry{ASR $\rightarrow$ ASR}
\addlegendentry{LSTM}


\legend{}

\end{axis}
\end{tikzpicture}
}

\\

\multicolumn{2}{c}{ \ref{leg} }

\end{tabular}
}
\caption{Forward and Backpropagation of different RNNs on a synthetic task designed to vary the length of the input sequences from $500$ to $9,000$ time steps. The original Li-GRU is a raw PyTorch implementation boosted with the native PyTorch Just-in-Time compilation. The Li-GRU 2.0 benefits from custom CUDA kernels to speed up the training. The LSTM is the official PyTorch implementation following CuDNN. The Li-GRU 2.0 is, on average, five times faster than the publicly available Li-GRU implementation, enabling realistic training on much larger datasets. The LSTM remains the fastest implementation due to the use of CuDNN. 
} \label{fig:perf_benchmark}
\end{center}
\end{figure*}


==> resources/curve_commonvoice.tex <==

\begin{figure*}[!th]
\begin{center}
\scalebox{0.89}{
\begin{tabular}{c, c}

\begin{tikzpicture}
\begin{axis}[
    width=10cm, height=5cm,   % size of the image
    grid = major,
    grid style={dashed, gray!30},
    xmin=1,   % start the diagram at this x-coordinate
    xmax=50,  % end  the diagram at this x-coordinate
    ymin=7,   % start the diagram at this y-coordinate
    ymax=20,  % end  the diagram at this y-coordinate
    axis background/.style={fill=white},
    tick align=outside,
    xtick={1,5,10,15,20,25,30, 35, 40, 45, 50},
    ytick={6, 8, 10, 12, 14, 16, 18, 20},
    mark repeat={600},
    ylabel near ticks,
    ylabel={Word Error Rate \% },
    xlabel near ticks,
    xlabel style={text width=5cm},
    xlabel style={align=center},
    xlabel={Epochs \\ CommonVoice IT (dev)},
    legend pos=north est,
    legend columns=1,
    legend style={
                    % the /tikz/ prefix is necessary here...
                    % otherwise, it might end-up with `/pgfplots/column 2`
                    % which is not what we want. compare pgfmanual.pdf
            /tikz/column 2/.style={
                column sep=2pt,
            },
    }
    ]

\addplot+[mark=none, name path global=ligru_layernorm,color=cyan,line width=1pt] file {resources/cv_ligru_50M_layernorm_it.txt};%\addlegendentry{ASR $\rightarrow$ ASR}
\addlegendentry{LiGRU Layernorm 50M}

\addplot+[mark=none,name path global=transformer,color=purple,line width=1pt] file {resources/cv_lstm_it.txt};%\addlegendentry{ASR $\rightarrow$ ASR}
\addlegendentry{LSTM 150M}

\addplot+[mark=none,name path global=transformer,color=orange,line width=1pt] file {resources/cv_ligru_150M_layernorm_it.txt};%\addlegendentry{ASR $\rightarrow$ ASR}
\addlegendentry{LiGRU Layernorm 150M}


%\addplot+[mark=none,name path global=transducer,color=orange,line width=1pt] file {resources/cv_transducer.txt};%\addlegendentry{ASR $\rightarrow$ ASR}

% 80% curves

\addplot+[only marks, color=orange, mark=*, mark options={draw=orange, fill=orange}] coordinates {
		(40, 9.52)
	}node[pin=200:{$9.52\%$}]{};



% resultats_DECODA_SANS_IVECTORS_DEV_corpus_RES_RES_RES_FALSE_EFR_2IT.txt 0.7952457142857122
% MEDIANE : 0.794285714285714 A LA POSITION 250.5 SUR 500


\end{axis}
\end{tikzpicture}

&

\begin{tikzpicture}
\begin{axis}[
    width=10cm, height=5cm,   % size of the image
    grid = major,
    grid style={dashed, gray!30},
    xmin=1,   % start the diagram at this x-coordinate
    xmax=25,  % end  the diagram at this x-coordinate
    ymin=7,   % start the diagram at this y-coordinate
    ymax=20,  % end  the diagram at this y-coordinate
    axis background/.style={fill=white},
    tick align=outside,
    xtick={1, 5, 10, 15, 20, 25},
    ytick={6, 8, 10, 12, 14, 16, 18, 20},
    mark repeat={600},
    ylabel near ticks,
    ylabel={Word Error Rate \% },
    xlabel near ticks,
    xlabel style={text width=5cm},
    xlabel style={align=center},
    xlabel={Epochs \\ CommonVoice FR (dev)},
    legend pos=north est,
    legend columns=1,
    legend style={
                    % the /tikz/ prefix is necessary here...
                    % otherwise, it might end-up with `/pgfplots/column 2`
                    % which is not what we want. compare pgfmanual.pdf
            /tikz/column 2/.style={
                column sep=2pt,
            },
    }
    ]


\addplot+[mark=none,name path global=transformer,color=purple,line width=1pt] file {resources/cv_lstm_fr.txt};%\addlegendentry{ASR $\rightarrow$ ASR}
\addlegendentry{LSTM 150M}

\addplot+[mark=none,name path global=transformer,color=orange,line width=1pt] file {resources/cv_ligru_150M_layernorm_fr.txt};%\addlegendentry{ASR $\rightarrow$ ASR}
\addlegendentry{LiGRU Layernorm 150M}


%\addplot+[mark=none,name path global=transducer,color=orange,line width=1pt] file {resources/cv_transducer.txt};%\addlegendentry{ASR $\rightarrow$ ASR}

% 80% curves

% speechbrain.utils.train_logger - Epoch loaded: 50 - test loss: 1.17, test CER: 3.05, test WER: 10.05


\end{axis}
\end{tikzpicture}


\end{tabular}
}

\caption{}
\end{center}
\end{figure*}


==> resources/curve_librispeech.tex <==

\begin{figure*}[!th]
\scalebox{0.89}{
\begin{tabular}{c}

\begin{tikzpicture}
\begin{axis}[
    width=10cm, height=5cm,   % size of the image
    grid = major,
    grid style={dashed, gray!30},
    xmin=1,   % start the diagram at this x-coordinate
    xmax=15,  % end  the diagram at this x-coordinate
    ymin=3,   % start the diagram at this y-coordinate
    ymax=15,  % end  the diagram at this y-coordinate
    axis background/.style={fill=white},
    tick align=outside,
    xtick={0, 1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14, 15},
    ytick={6, 8, 10, 12, 14, 16, 18, 20},
    mark repeat={600},
    ylabel near ticks,
    ylabel={Word Error Rate \% },
    xlabel near ticks,
    xlabel style={text width=5cm},
    xlabel style={align=center},
    xlabel={Epochs \\ LibriSpeech (dev)},
    legend pos=north est,
    legend columns=1,
    legend style={
                    % the /tikz/ prefix is necessary here...
                    % otherwise, it might end-up with `/pgfplots/column 2`
                    % which is not what we want. compare pgfmanual.pdf
            /tikz/column 2/.style={
                column sep=2pt,
            },
    }
    ]

\addplot+[mark=none, name path global=ligru_layernorm,color=cyan,line width=1pt] file {resources/cv_ligru_50M_librispeech.txt};%\addlegendentry{ASR $\rightarrow$ ASR}
\addlegendentry{LiGRU Layernorm 70M}




%\addplot+[mark=none,name path global=transducer,color=orange,line width=1pt] file {resources/cv_transducer.txt};%\addlegendentry{ASR $\rightarrow$ ASR}

% 80% curves

\addplot+[only marks, color=cyan, mark=*, mark options={draw=cyan, fill=cyan}] coordinates {
		(8, 6.53)
	}node[pin=200:{$6.53\%$}]{};




% resultats_DECODA_SANS_IVECTORS_DEV_corpus_RES_RES_RES_FALSE_EFR_2IT.txt 0.7952457142857122
% MEDIANE : 0.794285714285714 A LA POSITION 250.5 SUR 500


\end{axis}
\end{tikzpicture}



\end{tabular}
}

\caption{}
\end{figure*}

